Implicit bias of any algorithm: bounding bias via margin

Consider $n$ points $x_1,\ldots,x_n$ in finite-dimensional euclidean space, each having one of two colors. Suppose there exists a separating hyperplane (identified with its unit normal vector $w)$ for the points, i.e a hyperplane such that points of same color lie on the same side of the hyperplane. We measure the quality of such a hyperplane by its margin $\gamma(w)$, defined as minimum distance between any of the points $x_i$ and the hyperplane. In this paper, we prove that the margin function $\gamma$ satisfies a nonsmooth Kurdyka-Lojasiewicz inequality with exponent $1/2$. This result has far-reaching consequences. For example, let $\gamma^{opt}$ be the maximum possible margin for the problem and let $w^{opt}$ be the parameter for the hyperplane which attains this value. Given any other separating hyperplane with parameter $w$, let $d(w):=\|w-w^{opt}\|$ be the euclidean distance between $w$ and $w^{opt}$, also called the bias of $w$. From the previous KL-inequality, we deduce that $(\gamma^{opt}-\gamma(w)) / R \le d(w) \le 2\sqrt{(\gamma^{opt}-\gamma(w))/\gamma^{opt}}$, where $R:=\max_i \|x_i\|$ is the maximum distance of the points $x_i$ from the origin. Consequently, for any optimization algorithm (gradient-descent or not), the bias of the iterates converges at least as fast as the square-root of the rate of their convergence of the margin. Thus, our work provides a generic tool for analyzing the implicit bias of any algorithm in terms of its margin, in situations where a specialized analysis might not be available: it is sufficient to establish a good rate for converge of the margin, a task which is usually much easier.

==> analysis.tex <==
\section{Tools and full proof of the main result}
% The ideas used in the proofs are interesting in their own right; we believe the might find use in proofs other results elsewhere.
% on the unit-sphere $\mathbb S_{m-1}$.

\input{nonsmooth.tex}

==> deep.tex <==
\section{Implicit bias of multi-layer linear models}
\label{sec:deep}
Let $L \ge 1$ and $m_0,m_1,\ldots,m_L$ be positive integers with $m_0=m$ (the input dimension) and $m_L=1$ (the output dimension). A deep linear network is a function of the form
$$
\mathbb R^m \to \mathbb R,\;\x \mapsto \sign(\x^T\W_1\ldots\W_L) \in \{\pm 1\}.
$$
The matrix $\W_l \in \mathbb R^{m_l \times m_{l-1}}$ is the weights matrix of the $l$th layer. The tuple $\W=(\W_1,\ldots,\W_L)$ are the parameters of the network.
Note that the special case $L=1$ corresponds to simple linear models (only one layer).
As before, let $\ma$ be $n \times m$ matrix with $i$th row $a_i = -y_i \x_i$. Also, as before, since the classification of the model is independent of the norm of the weights matrices, the margin-maximization problem can be conviniently written as
\begin{eqnarray}
\overline{\gamma}_n := \max_{\|\W_1\|_{\fro} =1} \ldots \max_{\|\W_L\|_{\fro}=1}\min_{i \in [n]}\ma_i^\top\W_1\ldots\W_L
\end{eqnarray}
We start with the following basic Lemma.
\begin{restatable}{lm}{}
It holds that $\overline{\gamma}_n = \min_{\q \in \Delta_{n-1}}\|\A^\top \q\|_2$.
\label{lm:deepgamma}
\end{restatable} 
\begin{proof}
Using the elementary fact that $\max_{\|\Y\|_{\fro}  = 1}\|\B^\top \z\|_2 = \|\z\|_2$ repeatedly, we have
\begin{eqnarray*}
\begin{split}
\overline{\gamma}_n  &:= \max_{\|\W_1\|_{\fro} =1} \ldots \max_{\|\W_L\|_{\fro}=1}\min_{i \in [n]}\ma_i^\top\W_1\ldots\W_L\\
&=\max_{\|\W_1\|_{\fro} =1} \ldots \max_{\|\W_L\|_{\fro}=1}\min_{\q \in \Delta_{n-1}}\A^\top\q\W_1\ldots\W_L\\
&= \min_{\q \in \Delta_{n-1}}\max_{\|\W_1\|_{\fro} =1} \ldots \max_{\|\W_L\|_{\fro}=1}\A^\top\q\W_1\ldots\W_L\\
&= \min_{\q \in \Delta_{n-1}}\max_{\|\W_1\|_{\fro} =1} \ldots \max_{\|\W_L\|_{\fro}=1}\W_L^\top\ldots\W_1^\top(\A^\top\q)\\
&= \min_{\q \in \Delta_{n-1}}\max_{\|\W_1\|_{\fro} =1} \ldots \max_{\|\W_{L-1}\|_{\fro}=1}\|\W_{L-1}^\top\ldots\W_1(\A^\top\q)\|_2\\
&\quad\vdots\\
&= \min_{\q \in \Delta_{n-1}}\|\A^\top \q\|_2,
\end{split}
\end{eqnarray*}
as claimed.
\end{proof}
\begin{restatable}{rmk}{}
As should have been expected, the above lemma reveals that the maximum margin of a linear model does not depend on the the depth (i.e $L$) or architecture (i.e layer widths $m_l$). Thus, depth can only play a role with regards to optimization (not statistics).
\end{restatable}
Let $\opt^{\mathrm{deep}}_n := \{\W \mid \|\W_l\|_{\fro} = 1\;\forall l \in [L],\;\gamma_n(\W) = \overline{\gamma}_n\}$ be the set of all normalized max-margin multi-layer linear models with layer widths $m=m_0 \to m_1 \to \ldots \to m_L=1$. The following result is one of our main contributions.
\begin{restatable}[Error bound for deep linear networks]{lm}{}
For any instance of model parameters $\W = (\W_1,\ldots,\W_L)$ which are normalized, i.e $\|\W_l\|_{\fro} = 1$ for all $l \in [L]$. If $\gamma_n(\W) \ge 0$, we have
\begin{eqnarray}
\dist(\W,\opt^{\mathrm{deep}}_n) \le \frac{2}{\sqrt{L}}\cdot\left(1-\frac{\gamma_n(\W)}{\overline{\gamma}_n}\right)^{1/2}.
\end{eqnarray}
\label{thm:deepdist}
\end{restatable}

\subsection{The differential geometry of the parameter space of deep linear networks}
\begin{restatable}[Subdifferential on manifold]{thm}{}
Given a riemannian manifold $M$ embedded in $\mathbb R^r$ and a function $G:\mathbb R^r \to \mathbb R$, let $F$ be the restriction of $G$ on $M$. If $G$ is (Fr\'echet)-subdifferentiable at a point $\w \in M$, then so is $F$ (w.r.t the geometry of $M$), and its subdifferential is given by
$$
\partial F(\mathbf w) = \{\proj_{T_\mathbf w M}(\mathbf w^\star) \mid \mathbf w^\star \in \partial g(\mathbf w)\} \subseteq T_{\mathbf w} M,
$$
where $\proj_{T_{\mathbf w} M}:\mathbb R^r \to T_{\mathbf w}M$ is tangent space projection map at $\w$.
\label{prop:subdiffman}
\end{restatable}
The following elementary Lemma will be very useful.
\begin{restatable}[Retraction map of hyper-sphere]{lm}{}
For any positive integer $r$, we have the formular
$\proj_{T_\w\mathbb S_{r-1}}(\w^\star) = \proj_{\w^\perp}(\w^\star)= \w^\star-\langle \w^\star,\w\rangle \w,\;\forall \w \in \mathbb S_{r-1},\w^\star \in \mathbb R^r$.
\label{lm:retractsphere}
\end{restatable}

\paragraph{A manifold view of the parameter space.} For any layer index $l \in L$, of the deep linear network, let $N_l := m_{l-1}m_l$. The parameter space for the model can be succinctly written as
$$
\mathcal M = \{\W=(\W_1,\ldots,\W_L) \mid \W_l \in \mathbb R^{m_{l-1} \times m_l},\; \|\W_l\|_{\fro} = 1\;\forall l \in [L]\}.
$$
This is a $(\sum_{l=1}^{L}N_l-L)$-dimensional riemannian manifold embedded in $\Pi_{l=1}^{L}\mathbb R^{m_{l-1} \times m_l}$, which can be itself seen as a $\Pi_{l=1}^{L}N_l$-dimensional euclidean space with the natural inner-product given by $\langle \W,\widetilde{\W}\rangle := \sum_{l=1}^L\trace( \W_l\widetilde{\W_l}^\top)$.
Importantly, factorizes as a product of $L$ simpler riemannian manifolds,
$\mathcal M = \Pi_{l=1}^{L}\mathbb S_{m_{l-1}m_{l}-1}$.
 For example, when $L=2$, $m=m_0=1$, and $m_1=2$, this space is just the two-dimensional torus (doughnut) $\mathbb T_2 := \mathbb S_1 \times \mathbb S_1$.
 The tangent space on $\mathcal M$ at a point $\W=(\W_1,\ldots,\W_L)$ factorizes as into $L$ components like so
$T_{\W}\mathcal M = \prod_{l=1}^{L}T_{\W_l}\mathbb S_{N_l-1}$.
This means that the projection map for $\mathcal M$ is separable (i.e can be applied component wise), i.e
\begin{eqnarray}
\proj_{T_\W \mathcal M}(\W') = (\proj_{T_{\W_l}\mathbb S_{N_l-1}}(\W_l'))_{l \in [L]},\;\forall \W \in \mathcal M,\W' \in \Pi_{l=1}^L\mathbb R^{m_{l-1}\times m_l}.
\label{eq:projfactorize}
\end{eqnarray}
% For our margin-maximizaiton problem, our model space can be identified with $\mathcal M$, embedding in the  finite-dimensional euclidean space $\mathbb R^{m \times k} \times \mathbb R^k$ (equipped with Frobenius inner-product).
\begin{figure}[!h]
\centering
\begin{tikzpicture}
\centering
    \begin{axis}[hide axis]
       \addplot3[surf,
       colormap/cool,
       samples=20,
       domain=0:2*pi,y domain=0:2*pi,
       z buffer=sort]
       ({(2+cos(deg(x)))*cos(deg(y+pi/2))}, 
        {(2+cos(deg(x)))*sin(deg(y+pi/2))}, 
        {sin(deg(x))});
    \end{axis}
\end{tikzpicture}
\caption{Showing the 2-dimensional torus $\mathbb T_2=\mathbb S_1 \times \mathbb S_1$ as a riemannian manifold embedded in $\mathbb R^3$. This corresponds to the parameter space of a two-layer 1-dimensional linear model $1 \to 2 \to 1$.}
\end{figure}
\subsection{Proof of Theorem \ref{thm:deepdist}}
We are now ready to give a complete proof of Theorem \ref{thm:deepdist}.
\begin{proof}[Proof of Theorem \ref{thm:deepdist}]
The proof mimics the proof of Theorem \ref{thm:gold}, except for nontrivial difficulties due to the composition of multiple layers.
Consider the auxiliary function $F:\prod_{l=1}^{L}\mathbb R^{m_{l-1} \times m_{l}} \to \mathbb R \cup \{+\infty\}$ defined by 
$$
F(\W) := \begin{cases}-\gamma_n(\W)=\max_{i \in [n]}f_i(\W_1),&\mbox{ if }\W \in \mathcal M,\\
+\infty,&\mbox{ else}\end{cases}
$$
where $f_i:\prod_{l=1}^{L}\mathbb R^{m_l \times m_{l-1}} \to \mathbb R$ is the multilinear function defined by $f_i(\W):=\ma_i^\top \W_1\ldots\W_L$.

\emph{Step 1: Subdifferential of $F$.} Note that $f_i$ is differentiable with gradient $\nabla_{\W_l}f_i=\U_{l-1}^\top \ma_i \V_{l+1}^\top$, where $\U_l := \Pi_{j=1}^{l}\W_{j}$ and $\V_l := \Pi_{j=l}^L\W_j$. Let $\W \in \mathcal M$. Mindful of the cyclic invariance of trace and definition of the $\U_{l-1}$ and $\V_{l+1}$, for all $i \in [n]$ and $l \in [L]$, we have
    \begin{eqnarray}
    \begin{split}
    %\langle \U_{l-1}^\top\ma_i\V_{l+1}^\top,\W_l\rangle_{\fro} &:=
    \trace(\U_{l-1}^\top\ma_i\V_{l+1}^\top\W_l^\top)=\trace(\ma_i^\top\W_1\ldots\W_L)
    =:f_i(\W).
    \end{split}
    \label{eq:cyclic}
    \end{eqnarray}
% \begin{eqnarray}
% \nabla_{\W_l}f_i=\U_{l+1}^\top \ma_i \V_{l+1}^\top = \begin{cases}\ma_i\W_L^\top\ldots\W_2^\top,&\mbox{ if }l=1,\\
% \W_{l-1}^\top\ldots\W_2^\top\W_1^\top\ma_i\W_L^\top\ldots\W_{l+1}^\top,&\mbox{ if }2 \le l \le L-2,\\
% \W_{L-1}^\top\ldots\W_1 ^\top\ma_i,&\mbox{ if }l=L.
% \end{cases}
% \end{eqnarray}

Let $I (\W) := \{i \in [n] \mid f_i(\W) = F(\W)\}$ be the indices of the "support vectors" at $\W$ and let $\Delta_{n-1}(I(\W)) := \{\q \in \Delta_{n-1} \mid \sum_{i \in I(\W)}q_i = 1\}$ be the face of $\Delta_{n-1}$ spanned by these indices / vertices. Using Lemma \ref{lm:subdiffmax} and Theorem \ref{prop:subdiffman}, we compute the subdifferential of $F$ at $\W$ as 
\begin{eqnarray}
\label{eq:subdiffman}
\begin{split}
\partial F(\W) = % &= \left\{{\scriptstyle\sum}_{i=1}^n q_i \nabla_{\mathcal M} (\ma_i\U\mv) \mid \q \in \Delta_{n-1}(I(\W))\right\}\\
&=\left\{\proj_{T_\W\mathcal M}(({\scriptstyle\sum}_{i=1}^n q_i\U_{l-1}^\top\ma_i\V_{l+1}^\top)_{l \in L})\mid \q \in \Delta_{n-1}(I(\W))\right\}\\
&=\left\{(\proj_{T_{\W_l}\mathbb S_{N_l-1}}({\scriptstyle\sum}_{i=1}^n q_i\U_{l-1}^\top\ma_i\V_{l+1}^\top))_{l \in L}\mid \q \in \Delta_{n-1}(I(\W))\right\}\\
&=\left\{(\W_l'(\q))_{l \in [L]}\mid \q \in \Delta_{n-1}(I(\W))\right\}\\
\end{split}
\end{eqnarray}
where the second equality is due to \eqref{eq:projfactorize}, the third is due to Lemma \ref{lm:retractsphere} and $\W_l'(\q) \in T_{\W_l}\mathbb S_{N_l-1}$ is defined by
$\W_l'(\q) := {\scriptstyle\sum}_{i=1}^n q_i\U_{l-1}^\top \ma_i\V_{l+1}^\top-{\scriptstyle\sum}_{i=1}^nq_i\trace(\U_{l-1}^\top\ma_i\V_{l+1}^\top,\W_l^\top)\W_l$.
Thanks to \eqref{eq:cyclic}, for all $i \in I(\W)$ and $l \in [L]$, we can further simplify
\begin{eqnarray}
\W_l'(\q) = {\scriptstyle\sum}_{i=1}^n q_i\U_{l-1}^\top \ma_i\V_{l+1}^\top - {\scriptstyle\sum}_{i=1}^n f_i(\W)\W_l={\scriptstyle\sum}_{i=1}^n q_i\U_{l-1}^\top \ma_i\V_{l+1}^\top - F(\W)\W_l.
\label{eq:simplecyclic}
\end{eqnarray}

\emph{Step 2: Strong slope lower-bound for $F$.} For any $\W \in \mathcal M$, we compute
\begin{eqnarray*}
\begin{split}
\|\partial F(\W)\|^2 &= \inf_{\q \in \Delta_{n-1}(I(\W))}\sum_{l=1}^L\|\W'_l(\q)\|_{\fro}^2\\
&=\inf_{\q \in \Delta_{n-1}(I(\W))}{\scriptstyle\sum}_{l=1}^L\left(\left\|\U_{l-1}^\top\A^\top\q\V_{l+1}^\top\right\|_{\fro}^2-F(\W)^2\right),\text{ by \eqref{eq:simplecyclic}}\\
&\ge \inf_{\q \in \Delta_{n-1}(I(\W))}{\scriptstyle\sum}_{l=1}^L\left(\left\|\U_{l-1}^\top\A^\top\q\V_{l+1}^\top\W_l^\top\right\|_{\fro}^2-F(\W)^2\right),\text{ since }\|\W_l^\top\|_{\fro}=1\\
&=\inf_{\q \in \Delta_{n-1}(I(\W))}L\cdot((\A^\top\q\W_1\ldots\W_L)^2-F(\W)^2),\text{ by cyclic invariance of trace}\\
&\ge L\cdot\inf_{\q \in \Delta_{n-1}}((\A^\top\q\W_1\ldots\W_L)^2-F(\W)^2),\text{ because }\Delta_{n-1}(I(\W)) \subseteq \Delta_{n-1}\\
&=L\cdot(\overline{\gamma}_n^2-F(\W)^2),\text{ by Lemma \ref{lm:deepgamma} and the fact that }\overline{\gamma}_n >0\text{ by assumption}\\
&= L\cdot(\overline{\gamma}_n-F(\W))(F(\W)+\overline{\gamma}_n)\\
&= L\cdot(\overline{\gamma}_n+\gamma_n(\W))(F(\W)-\min F),
% \text{ since }F(\W)=-\gamma_n(\W)\text{ and }-\overline{\gamma}_n=\min F
\text{ by definition of }F.
\end{split}
\label{eq:step2}
\end{eqnarray*}

Thus, if $\gamma(\W) \ge 0$, then $\|\partial F(\W)\|^2 \ge L\overline{\gamma}_n\cdot (F(\W)-\min F)$ which is a KL-inequality with exponent $\theta=1/2$ and weight $\alpha = L\overline{\gamma}_n$. It then suffices to invoke Proposition \ref{prop:nonlinearhoffman} with $M=(\mathcal M,d_{geo})$, $\alpha=L\overline{\gamma}_n$, and $\theta=1/2$ to get the result.
\end{proof}

==> hadamard.tex <==
\begin{restatable}[Hadamard-differentiability]{df}{}
Let $M=(M,\|\cdot\|)$ be a Banach space. A function $f:M \to \mathbb R$ is said to be Hadamard-differentiable at the point $\w \in M$ and in the direction $\bu \in M\setminus\{\bO\}$ if the following limit exists
$$
\liminf_{t \to 0^+,\; \mv \to \bu}\frac{f(\w + t\mv)-f(\w)}{t}.
$$
The value of the limit is then called the Hadamard derivative of $f$ at $\w$, in the direction $\bu$, denoted $f'(\w;\bu)$. $f$ is said to be Hadamard-differentiable at $\w$ if it is Hadamard-differentiable at $\w$ in every direction.
\end{restatable}

==> nonsmooth.tex <==
\subsection{Nonsmooth analysis in Banach and metric spaces}
\label{sec:nonsmooth}
% We start with a swift digression to nonsmooth analysis, the final purpose being to arrive at
%\eqref{eq:proofmachine0}, and ultimately a proof of our main result (Theorem
% \ref{thm:main}).
% The material developed here is valid for any Banach space $M=(M,\|\cdot\|)$ with topological dual $M^\star=(M^\star,\|\cdot\|_\star)$; recall that this is made of all bounded linear maps $M \to \mathbb R$. The self-dual finite-dimensional euclidean case $M=(\mathbb R^m,\|\cdot\|_2)$ is only a peculiar instance of this general setup.
% \begin{restatable}[Subdifferential, see ~\cite{rockafellar}]{df}{}
% Given an  function $f:M \to \mathbb R \cup \{\infty\}$ and a point $\w \in M$, the subdifferential of $f$ at $\w$, denoted $\partial f(\w)$, is defined by
% $$
% \partial f(\w) := \{\x \in M^\star \mid f(\w') \ge f(\w) + \langle \x,\w'-\w\rangle,\;\forall \w' \in M\},
% $$
% $f$ is said to be subdifferentiable at $\w$ just in case $\partial f(\w) \ne \emptyset$.%  In this case, we define the subdifferential norm of $f$ at $\w$, denoted $\|\partial f(\w)\|_\star$, by
% % $$
% % \|\partial f(\w)\|_\star := \dist(\bO,\partial f(\w)) =: \inf\{\|\x\|_\star \mid \x \in \partial f(\w)\}.
% % $$
% \end{restatable}

% \todo{It appears we no longer need the concept of strong slopes, just subdifferentials of minimal norm!}

% The concept of \emph{strong-slope}~\cite{degiorgi80} will play a fundamental role in our framework.
% \begin{restatable}[The "strong slope" of a function at a point]{df}{}
% Let $M=(M,d)$ be a metric space and $f:M \to (-\infty,+\infty]$ be a function. The strong slope of $f$ at the point $\w \in M$, denoted $\sslope f(\w)$, is defined by
% \begin{eqnarray}
%   \sslope f(\w) := \limsup_{\w' \to \w}\frac{(f(\w)-f(\w'))_+}{d(\w',\w)},
%   \label{eq:strongslope}
% \end{eqnarray}
% with the convention that $\sslope f(\w) = \infty$ if $f(\w) = \infty$.
% \label{df:strongslope}
% \end{restatable}

% % \input{hadamard.tex}

% \begin{restatable}{rmk}{}
% \label{rmk:lips}
% The following standard facts should be noted about the concept of strong slope. 
% \begin{itemize}
% \item {\bfseries Our notation.} Note that \cite{nonlinearhoffman} uses the notation $|\nabla f|(\w)$ to denote the
%   strong-slope of $f$ at $\w$. We prefer to use the notation $\sslope f(\w)$ instead,
%   which avoids the deceptive "$\nabla$" which may be confused with gradients in
%   the usual sense.
% \item {\bfseries Link with Lipschitz semi-norm.} % In the special case where $M=(M,\|\cdot\|)$ is a Banach space and $f$ is a
%   % convex function on it,
%  Observe that if $f$ does not attain a local minimum at the point $\w \in M$, then
% \begin{eqnarray}
% \sslope f(\w) \le \underset{\w' \in M,\;\w' \ne
%   \w}{\sup}\;\frac{f(\w')-f(\w)}{d(\w',\w)},
%   \end{eqnarray}
%   and so $
% \sslope f(\w) \le \|f\|_{\Lip}$, where $\|f\|_{\Lip}$ is the Lipschitz semi-norm of $f$ defined by 
% \begin{eqnarray}
% \|f\|_{\Lip}:= \underset{\w',\w \in M,\;\w' \ne \w}{\sup}\;\frac{f(\w')-f(\w)}{d(\w',\w)}.
%   \label{eq:lipsconstant}
% \end{eqnarray}
% % \item In case $M=(M,\|\cdot\|)$ is a Banach space and
% %   $f$ is sub-differentiable at $\w$\footnote{Meaning that the subdifferential of $f$ at
% %     $\w$, namely the set $\{\mv \in M \mid f(\z) \ge f(\w) +
% %     \mv^\top(\z-\w),\;\forall \z \in M\}$, is nonempty.} we have
% %   $\sslope f(\w) := \inf_{\mv \in \partial f(\w)}\|\mv\|$. Further, if $f$ is
% %   Fr\'echet-differentiable at $\w$, then $\sslope f(\w) = \|\nabla f(\w)\|_*$.
% \item {\bfseries Link with subgradients.} In particular, if $M = (M,\|\cdot\|)$ is a normed vector-space and $f: M \to (-\infty,+\infty]$ is an  function, then
% \begin{eqnarray}
% \sslope f(\w) \le \|\partial f(\w)\|_\star := \dist(\bO,\partial f(\w)) := \inf\{\|\x\|_\star \mid \x \in \partial f(\w)\},
% \label{eq:subdiffminnorm}
% \end{eqnarray}
% where $\partial f(\w)$ is the subdifferential of $f$ at $\w$ defined by $\partial f(\w) := \{\x \in M^\star \mid f(\w') \ge f(\w) + \langle \x,\w'-\w\rangle,\;\forall \w' \in M\}$, with $M^\star = (M^\star,\|\cdot\|_\star)$ being the topological dual of $M$.
% Moreover, if $f$ is convex, then equality holds in \eqref{eq:subdiffminnorm}. See ~\cite[Proposition 5.2]{hoffmanlsc}
% \end{itemize}
% \label{lm:convexslope}
% \end{restatable}

% \begin{restatable}[Strong slopes via subdifferentials]{prop}{}
% Let $M = (M,\|\cdot\|)$ be a real normed vector-space and let $f: M \to (-\infty,+\infty]$ be a lower-semicontinuous function. Then, we have the upper-bound
% $$
% \sslope f(\w) \le \dist(\bO,\partial f(\w)) := \inf\{\|\mv\| \mid \mv \in \partial f(\w)\},
% $$
% with equality if $f$ is convex. On the other hand, if $f$ is Hadamard-differentiable at $\w$,
% then
% $$
% \sslope f(\w) \ge \sup_{\|\bu\| \le 1} -f'(\w;\bu)
% $$
% \end{restatable}
The following fundamental theorem from ~\cite{hoffmanlsc} will be an essential tool for us.
%\begin{mdframed}[backgroundcolor=black!10,rightline=false,leftline=false]
\begin{restatable}[Nonlinear error-bound via Kurdyka-\L{}ojasiewicz]{prop}{}
Let $M$ be a complete metric space and $f:M \to \mathbb R\cup\{+\infty\}$ be a proper l.s.c function which satisfies a KL-inequality around $\w_0$ with exponent $\theta>0$ and modulus $\alpha>0$.
Then, if $a := f(\w)$,  we have the error-bound
\begin{eqnarray}
\dist(\w,\{f \le a\}) \ge \frac{(f(\w)-a)^\theta}{\alpha},\;\forall \w \in M\text{ with } f(\w) > a.
\label{eq:nonlinearhoffman}
\end{eqnarray}
\label{prop:nonlinearhoffman}
\end{restatable}
% \end{mdframed}
% \begin{restatable}{rmk}{}
% The quantity $\|\partial f(\w)\|_\star$ is nothing but the \emph{strong slope} (see ~\cite{degiorgi80} for definition) of the function $f$ at the point $\w$. The concept of strong slope is definable for general nonconvex functions. In the case of convex functions functions, it is known to coincide with the definition of $\|\partial f(\w)\|_\star$. 
% There is a rich history surrounding results in the spirit of Proposition \ref{prop:nonlinearhoffman} above. For example, it
% has deep connections with the \emph{Kurdika-\L{}ojasiewicz theory} that has been
% very successful in analyzing the convergence of gradient-descent and proximal
% schemes in very general spaces (e.g \emph{Asplund} spaces).  The interested
% reader might want to consult ~\cite{hoffmanlsc,nonlinearhoffman,bolteOT} and there
% references therewithin.
% % \end{restatable}

% Proposition \ref{prop:nonlinearhoffman} has many interesting consequences. In
% particular, one immediately deduces that if $C$ is a nonempty subset of $M$
% such that $\|\partial f(\w)\|_\star \ge \alpha$ for every $\w \in C$ and for
% some $\alpha > 0$, then
% \begin{eqnarray}
% \dist(\w,\arg\min f) \ge \frac{(f(\w) - \min f)^\theta}{\alpha},\;\forall \w \in C.
% \label{eq:anyC}
% \end{eqnarray}
% \begin{mdframed}

% We conclude this detour with the following result which is one of our main
% contributions. Its a nontrivial corollary to Proposition
% \ref{prop:nonlinearhoffman}, which --in combination with \eqref{eq:anyC}-- will
% play an important role in our proof of Theorem \ref{thm:main}. Viz
% \begin{restatable}[Error analysis for piecewise-linear functions]{thm}{gold}
% Let $M$ be a (real) Hilbert space and let $\ma_1,\ldots,\ma_n \in M$. Consider the  concave
% function $g:M \to \mathbb R \cup \{-\infty\}$ defined by
% $$
% g(\w) := \begin{cases}\min_{i \in [n]} \langle \ma_i,\w\rangle,&\mbox{ if }\|\w\| = 1,\\
% -\infty,&\mbox{ else.}
% \end{cases}
% $$
% Suppose $\arg\max g \ne \emptyset$ and $\gamma := \max g > 0$. Then, for every $\w \in \{0 < g < \gamma\}$, it holds that
% \begin{eqnarray}
% \dist(\w,\arg\max g) \le 2\left(1 - \frac{g(\w)}{\gamma}\right)^{1/2}.
% \end{eqnarray}
% \label{thm:gold}
% \end{restatable}
% \begin{restatable}{rmk}{}
% Note that the assumption $\arg\max g \ne \emptyset$ is only needed in case of infinite-dimensional spaces (indeed, in finite-dimensions, closed balls are compact,  plus, it is an elementary fact that a continuous function on a compact set attains its maximum on the that set).
% \end{restatable}
% The proof of Theorem \ref{thm:gold} is instructive and is provided in the main manuscript.
For our proofs, we will need the following lemma is a direct consequence of the well-known Danskin-Bertsekas theorem for subdifferentials ~\cite[Proposition A.22]{bersekas}. See appendix for a proof.
\begin{restatable}[Subdifferential of maximum of $n$ functions]{lm}{danskinbertsekas}
Let  $M$ be a (real) Hilbert space and $f_1,\ldots,f_n:M \to \mathbb R \cup \{+\infty\}$ be convex functions and let $f$ be their pointwise maximum. Then for any $\w \in M$, we have the subdifferential identity
$$
\partial f(\w) = \conv(\cup_{i \in I(\w)} \partial f_i(\w)),
$$
where $I(\w) := \{i \in [n] \mid f_i(\w) = f(\w)\}$ is the subset of indices active at $\w$.
\label{lm:subdiffmax}
\end{restatable}
% Let $\mathbb B_M := \{\w \in M \mid \|\w\| \le 1\}$ be the unit-ball in $M$. We will also need the elementary result which is proven in the appendix.
% % \begin{restatable}[Subdifferential sum-rule]{lm}{}
% % Let $f_1,f_2:M \to \mathbb R \cup \{\infty\}$ be convex functions such that the relative interiors of their effective domains have a common point, i.e $\interel \dom f\cap \interel\dom f_2 \ne \emptyset$. Then the subdifferential of their sum $f := f_1 + f_2$ at any point $\w \in M$ is the Minkowski sum of the subdifferentials of $f_1$ and $f_2$ at $\w$. That is,
% % $\partial f(\w) = \partial f_1(\w) + \partial f_2(\w) := \{\w_2^\star + \w_2^\star \mid \w_k^\star \in \partial f_k(\w)\;k=1,2\}$.
% % \label{lm:subdiffsum}
% % \end{restatable}

% \begin{restatable}[Subdifferential of indicator of closed unit-ball]{lm}{ncone}
% Let $i_{\mathbb B_M}:M \to \mathbb R \cup \{\infty\}$ be the indicator function of the unit-ball of $\mathbb B_M$, defined by
% $$
% i_{\mathbb B_M}(\w) := \begin{cases}0,&\mbox{if }\w \in \mathbb B_M,\\
% +\infty,&\mbox{else.}
% \end{cases}
% $$
% If $\w \in M$ with $\|\w\| < 1$, then $\partial i_{\mathbb B_M}(\w) = \{\bO\}$.
% % := \mathcal N_{\mathbb B_M}(\w)$,
% %
% % equals the normal cone of $\mathbb B_M$ at $\w$ given by
% % $
% % \mathcal N_{\mathbb B_M}(\w) := \begin{cases}\{\bO\},&\mbox{ if }\|\w\| < 1,\\\mathbb R_+\w,&\mbox{ if }\|\w\| = 1,\\\emptyset,&\mbox{ otherwise.}
% % \end{cases}
% % $
% \label{lm:ncone}
% \end{restatable}

% \subsection{The (sub)differential geometry of the sphere $\mathbb S_{m-1}$}
\subsection{Proof of Theorems \ref{thm:gold} and \ref{thm:main}}
We start with a generic result computing subdifferentials of functions restricted unto manifolds.
\begin{restatable}[Subdifferential on manifold]{prop}{}
Given a riemannian manifold $M$ embedded in $\mathbb R^m$ and a function $F:\mathbb R^m \to \mathbb R$, let $f:(M,d_{geo}) \to \mathbb R$ be the restriction of $F$ on $M$. If $F$ is (Fr\'echet)-subdifferentiable at a point $\w \in M$, then so is $f$, and its subdifferential is given by
\begin{eqnarray}
\partial f(\mathbf w) = \{\proj_{T_\mathbf w M}(\mathbf w^\star) \mid \mathbf w^\star \in \partial F(\mathbf w)\} \subseteq T_{\mathbf w} M,
\end{eqnarray}
where $\proj_{T_{\mathbf w} M}:\mathbb R^m \to T_{\mathbf w}M$ is tangent space projection map at $\w$.
\label{prop:subdiffman}
\end{restatable}
The following elementary Lemma will be very useful.
\begin{restatable}[Tangent-space projection map for $\mathbb S_{m-1}$]{lm}{}
The following formula holds
$$
\proj_{T_\w\mathbb S_{m-1}}(\mv) = \proj_{\w^\perp}(\mv)= \mv-(\mv^\top\w) \w,\;\forall \w \in \mathbb S_{m-1},\mv \in \mathbb R^m.
$$
Moreover, $\|\proj_{T_\w\mathbb S_{m-1}}(\mv)\|^2 = \|\mv\|^2 - (\mv^\top\w)^2$.
\label{lm:retractsphere}
\end{restatable}
\begin{proof}
$\mathbb S_{m-1}$ is defined by the equation $\|\w\|^2 = 1$. At the point $\w$, the tangent space is the hyperplane with unit-normal vector $\w$. Therefore $T_\w\mathbb S_{m-1} = \w^\perp := \{\mv \in \mathbb R^m \mid \mv^\top\w = 0\}$. The formula for the projection operator $P_{T_\w\mathbb S_{m-1}}$ then follows from algebraic manipulations.
\end{proof}

We are now ready to proof Theorem \ref{thm:gold}.

\begin{proof}[Proof of Theorem \ref{thm:gold}]
Let $F:\mathbb R^m \to \mathbb R$ the extension of $f=-\gamma:\mathbb S_{m-1} \to \mathbb R$ to all of $\mathbb R^m$, defined by $F(\w') = \min_{i \in [n]}F_i(\w)$, where $f_i(\w'):=\ma_i^\top \w'$, for all $\w' \in \mathbb R^m$.
Note that each $F_i$ is differentiable and convex, with (Fr\'echet-)subdifferential equal to the singleton $\{\ma_i\}$.
 Thus, according to Lemma \ref{lm:subdiffmax}, the subdifferential of $F$ at $\w'$ is given by $\partial F(\w') = \conv\{\ma_1,\ldots,\ma_n\}$, where $I(\w') := \{i \in [n] \mid \ma_i^\top\w' =  f(\w')\}$ is the set of indices of the "support vectors" at $\w'$ and $\Delta_{n-1}(I(\w')) := \{\q \in \Delta_{n-1} \mid q_i = 0\;\forall i \not\in I(\w')\}$ be the face of the simplex $\Delta_{n-1}$, spanned by the vertices in $I(\w)$.
 
 Let $\w \in \mathbb S_{m-1}$ with $\gamma(\w)>0$. One computes
\begin{eqnarray*}
\begin{split}
    \|\partial f(\w)\|^2 &:= \inf \{\|\w^\star\| \mid \w^\star \in \partial f(\w)\}
    \\
    &= \inf_{\w^\star \in \partial F(\w)}\left\|\proj_{T_\w\mathbb S_{m-1}}(\w^\star)\right\|^2,\text{ by Proposition \ref{prop:subdiffman}}\\
    &= \inf_{\w^\star \in \partial F(\w)}\|\w^\star - (\w^\top\w^\star)\w\|^2=\inf_{\w^\star \in \partial F(\w)} \|\w^\star\|^2-\left(\w^\top\w^\star\right)^2,\text{ by Lemma \ref{lm:retractsphere}}\\
    &=\inf_{\q \in \Delta_{n-1}(I(\w))} \|{\scriptstyle\sum}_{i=1}^nq_i\ma_i\|^2-({\scriptstyle\sum}_{i=1}^nq_i\ma_i^\top\w)^2,\text{ since }\partial F(\w) = \conv\{\ma_1,\ldots,\ma_n\}\\
    &= \inf_{\q \in \Delta_{n-1}(I(\w))} \left\|{\scriptstyle\sum}_{i=1}^n q_i\ma_i\right\|^2 - \gamma(\w)^2,\text{ since }\ma_i^\top\w = \gamma(\w)\;\forall i \in I(\w)\\
    &\ge \inf_{\q \in \Delta_{n-1}}\left\|{\scriptstyle\sum}_{i=1}^n q_i\ma_i\right\|^2 -\gamma(\w)^2,\text{ because }\Delta_{n-1}(I(\w)) \subseteq \Delta_{n-1}\\
    &=\gammaopt^2-\gamma(\w)^2 = (\gammaopt+\gamma(\w))(\gammaopt-\gamma(\w))\\
    &\ge \gammaopt\cdot (\gammaopt-\gamma(\w)),\text{ because }\gamma(\w)>0\text{ by assumption}\\
    & =\gammaopt\cdot(f(\w)-\min f),\text{ by definition of }f
    \end{split}
    \end{eqnarray*}
% Now, let $\A \in M^n$ be matrix whose $i$th row is the vector $\ma_i \in M$.
Combining the above inequality with \eqref{eq:sslopebounds}, gives
$$
\sslope f(\w) \ge \liminf_{(\w',f(\w')) \to (\w,f(\w))}\|\partial f(\w')\| \ge \gammaopt^{1/2}\cdot (f(\w)-\min f)^{1/2}.
$$
Thus, the funciton $f$ satisfies a KL-inequality with exponent $\theta=1/2$ and modulus $\alpha=2/\sqrt{\gammaopt}$, as claimed.
% Now, fix $\epsilon \in (0,1)$. For $\w \in \mathbb B_M$, let $\w_\epsilon := (1-\epsilon)\w$. The proof is broken into several steps.

% \emph{Step 1: Bounding the strong slope $\|\partial f(\w_\epsilon)\|$.} Invoking the a special case of the "subdifferential sum-rule" ~\cite[Lemma 2]{verona2001} and the definition of $f$, we have $\partial f(\w) = \partial (\max_{i \in [n]}-\ma_i)(\w_\epsilon) + \partial i_{\mathbb B_{M}}(\w_\epsilon)$.
% But because $\|\w_\epsilon\| = 1-\epsilon < 1$, we have $\partial i_{\mathbb B_{M}}(\w_\epsilon) = \{\bO\}$ by Lemma \ref{lm:ncone}. % Indeed by definition of subdifferentials, $\bu \in \partial i_{\mathbb B_M}(\w_\epsilon) \implies \langle \bu,\w' - \w\rangle \le 0 \;\forall \w' \in \mathbb B_M \implies \|\bu\| \le \langle \bu,\w\rangle \le \|\bu\|\|\w\|$, which is only possible if $\bu = \b0$; on the other hand, $\bO \in \partial i_{\mathbb B_M}(\w_\epsilon)$ clearly.
% Thus $\partial f(\w) = \partial (\max_{i \in [n]}-\ma_i)(\w_\epsilon)$, and invoking Lemma \ref{lm:subdiffmax} then gives
% $$
% \partial f(\w_\epsilon) = \partial (\min_i (-\ma_i))(\w_\epsilon) =  \conv(\{-\nabla \ma_i(\w_\epsilon) \mid i \in I(\w_\epsilon)\}\} = \conv(\{-\ma_i \mid i \in I(\w_\epsilon)\},
% $$
% where $I(\w_\epsilon) := \{i \in [n] \mid \langle -\ma_i,\w_\epsilon\rangle = f(\w_\epsilon)\}$. Putting things together, one then computes
% \begin{eqnarray*}
% \begin{split}
% \|\partial f(\w_\epsilon)\| 
% &:= \inf \{\|\x\|_\star \mid \x \in \partial f(\w_\epsilon)\} = \inf\{\|\x\|_\star \mid \x \in \conv(\{-\ma_i \mid i \in I(\w_\epsilon)\}\}\\
%  &\ge \inf\{\|\x\|_\star \mid \x \in \mbox{conv}(\{-\ma_i \mid i \in [n]\}\},\text{ since infimum on larger set is smaller}\\
% &= \min_{\q \in \Delta_{n-1}}\|{\scriptstyle\sum}_{i=1}^nq_i\ma_i\|_\star = \min_{\q \in \Delta_{n-1}}\max_{\|\w'\| \le 1}{\scriptstyle\sum}_{i=1}^n q_i \langle \ma_i,\w'\rangle,\text{ by duality}\\
% &\ge \max_{\|\w\| \le 1}\min_{\q \in \Delta_{n-1}}{\scriptstyle\sum}_{i=1}^n q_i \langle \ma_i,\w'\rangle,
% \text{ because }\min\max \ge \max\min
% \\
% &=\max_{\|\w'\| \le 1}\min_{i \in [n]}\langle \ma_i,\w'\rangle,\text{ since min. of linear functional on simplex is attained at a vertex}\\
% &= \max_{\|\w'\| \le 1}g(\w') =: \max g =: \gamma >0,\text{ by definition of  }g.
% \end{split}
% \end{eqnarray*}
% Thus $\|\partial f(\w_\epsilon)\|_\star \ge \gamma:=\max g > 0$.

% \emph{Step 2: Bounding distance to maximizers.}
% Using Proposition \ref{prop:nonlinearhoffman} with $f=-g$ then gives
% \begin{eqnarray*}
% \begin{split}
% \dist(\w,\arg\max g) &\le \|\w-\w_\epsilon\| + \dist(\w_\epsilon,\arg\max g),\text{ by triangle inequality}\\
% &= \epsilon + \dist(\w_\epsilon,\arg\gamma),\text{ by definition of }\w_\epsilon\\
% &\le \epsilon + 1-\frac{g(\w_\epsilon)}{\gamma},\text{ by Proposition \ref{prop:nonlinearhoffman} and the fact that }\|\w_\epsilon\| = 1-\epsilon < 1\\
% &\le \epsilon + 1 - \frac{g(\w) - \epsilon\max_{i \in [n]} \|\ma_i\|_\star}{\gamma},\text{ because }g\text{ is }(\max_{i \in [n]}\|\ma_i\|_\star)\text{-Lipschitz}\\
% &= 1 - \frac{g(\w)}{\gamma} + \epsilon(1 + \frac{\max_{i \in [n]}\|\ma_i\|_\star}{\gamma}).
% \end{split}
% \end{eqnarray*}

% Finally, letting $\epsilon \rightarrow 0^+$ then gives $\dist(\w,\arg\max g) \le 1 - g(\w)/\gamma$ as claimed.
\end{proof}
\begin{proof}[Proof of Theorem \ref{thm:main}]
From Theorem \ref{thm:gold}, we know that the negative margin function $-\gamma$ satisfies a KL-inequality with exponent $\theta=1/2$ and modulus $\alpha=2/\sqrt{\gammaopt}$. The result then follows as upon invoking \ref{prop:nonlinearhoffman}.
\end{proof}

% \begin{restatable}{lm}{sslopemax}
% Let $M = (M,\|\cdot\|)$ be a real normed vector-space and consider continuously differentiable convex functions $f_1,\ldots,f_n: M \to \mathbb R$ with gradient maps $\nabla f_1,\ldots,\nabla f_i: M \to M^\star$. Then we have the lower-bound
% \begin{eqnarray}
% \sslope f (\w) \ge \sup_{\|\bu\| \le 1}\min_{i \in [n]}\nabla f_i(\w)^\top\bu,\;\forall \w \in M,
% \end{eqnarray}
% where $f := \max_{i \in [n]} f_i:M \to (-\infty,+\infty]$ is the point-wise maximum of the functions.
% \label{lm:sslopemax}
% \end{restatable}


% Indeed, for every $\w \in \mathbb S_{m-1}$, one computes\footnote{The derivative in $\mathbb R^m$ is $-y_i\x_i$. To get the derivative on $\mathbb S_{m-1}$ we need to project this onto the tangent space at $\w$. But } $\nabla f_i(\w) = -y_i\x_i$, and so by Lemma \ref{lm:sslopemax},
% \begin{eqnarray*}
% \begin{split}
% \sslope (-\gamma)(\w) = \sslope (\max_{i \in [n]}f_i)(\w)  &\ge \sup_{\|\bu\| \le 1}\min_{i \in [n]}-y_i\x_i^\top\bu\\
% &= \sup_{\bu \in \mathbb S_{m-1}}\min_{i \in [n]}y_i\x_i^\top\bu =: \gammaopt.
% \end{split}
% \end{eqnarray*}

% % The following result from ~\cite{nonlinearhoffman} gives an effective way to
% % lower-bound strong-slopes via Hadamadard derivatives, which are morally easier
% % to compute.
% % \begin{restatable}[Strong-slope lower-bound]{prop}{}
% % If $M$ is a Banach space and $f:M \to \mathbb R$ is
% % Hadamard-differentiable at a point $\w \in M$, then we have the
% % lower-bound
% % \begin{eqnarray}
% % \sslope f(\w) \ge \sup_{\|\bu\| \le 1} -f'(\w;\bu),
% % \label{eq:strongslopebound}
% % \end{eqnarray}
% % with equality if the space is finite-dimensional.
% % \label{prop:strongslopebound}
% % \end{restatable}

% The following result is from ~\cite[Proposition 2.1]{nonlinearhoffman}, and motivates the interest in the strong-slope operator $\sslope$ in the first place.
% \begin{restatable}[Master variational theorem]{prop}{}
% Let $M=(M,d)$ be a complete metric space and $U$ be a nonempty open subset of $M$. If $f:M \to \mathbb (-\infty,+\infty]$ is a lower-semicontinuous function, then % we have the following upper-bound
% \begin{eqnarray}
% \inf_{\w' \in U}\sslope f(\w')\cdot \dist(\w,M\setminus U) \le f(\w)-\min_{\w' \in U}f(\w'),\text{ for all }\w \in U.
% \end{eqnarray}
% \label{prop:hoffman}
% \end{restatable}
% There is a rich history surrounding results of the above type. For example, it
% has deep connections with the \emph{Kurdika-\L{}ojasiewicz theory} that has been
% very successful in analyzing the convergence of gradient-descent and proximal
% schemes in very general spaces (e.g \emph{Asplund} spaces).  The interested
% reader might want to consult ~\cite{nonlinearhoffman,bolteOT} and there
% references therewithin.

% We end this subsection with the following corollary which will be particularly useful for our purposes. It allows us to bound the distance between a point and the set of minimizers of a "nice" function.
% \begin{restatable}[Distance to maximizers]{cor}{myhoffman}
% Let $M=(M,d)$ be a complete metric space and let $C$ be a closed subset of $M$. Let $f:M
% \to (-\infty,+\infty]$ be a lower-semicontinuous and define $\arg\min f|_C := C \cap \arg\min f$ and $f|_C^\star := \min_{\w \in C}f(\w)$. Suppose $\sslope f(\w) \ge \alpha>0$ for some $\alpha>0$ and for all $\w \in M$ with $\w \not\in \arg\min f|_C$.
% Then % we have the following upper-bound
% \begin{eqnarray}
% \dist(\w,\arg\min f|_C) \le \frac{f(\w)-f|_C^\star}{\alpha},\text{ for all }\w \in M.
% \label{eq:hoffman}
% \end{eqnarray}
% \label{corr:myhoffman}
% \end{restatable}

% % \lorem
% % \begin{restatable}{rmk}{}
% Thus, uniform lower-bound on the strong-slope $\sslope f$ of the function $f$ gives us full control on the distance of every point to the set of minimizers $f$. This is precisely what we need for our analysis of the implicit bias of gradient-flow. % On the other hand, we know from Rmk. \ref{rmk:lips} that for convex
% % functions, the strong-slope $\sslope f(\w)$ is uniformly upper-bounded by the
% % Lipschitz semi-norm $f$ (defined in \eqref{eq:lipsconstant}), i.e $\|f\|_{\Lip} \ge \sslope f(\w)$, for every $\w$ which
% % is not a minimum point of $f$.
% % \end{restatable}

% \input{deep.tex}


==> old_blablabla.tex <==
Consider the following gradient-flow (aka continuous-time limit of gradient-descent) on $-\risk_n$
\begin{eqnarray}
\label{eq:gradflow}
\begin{split}
\frac{d\w(t)}{dt} &= \nabla \risk_n(\w(t)),\;\w(0) = \bO.
\end{split}
\end{eqnarray}
The initial condition $\w(0) = \b0$ is only for convenience and plays no crucial role in our results and proofs.
We will analyse the gradient-flow scheme \eqref{eq:gradflow} and show that its solution converges wit time, to a limit point (after normalization by norm) of $\opt_n$, at a rate $\mathcal O(1/t)$

The following is one of our main results. It can be extended to any exponential-tail loss function (as defined in ~\cite{soudry2017}). Viz
\begin{restatable}[$\mathcal O(1/t)$ convergence rate of the bias of gradient-flow]{thm}{}
  Let $\w_n(t)$ be a solution of \eqref{eq:gradflow} at time $t > 0$. Then, we have the the following bound
% {\bfseries (A) Convergence rate of margin:}
% \begin{eqnarray}
%   0 \le  \overline{\gamma}_n - \gamma_n(\widetilde{\w}_n(t)) \le \frac{\log
%   n}{\overline{\gamma}_n t}.
%   \label{eq:marginrate}
% \end{eqnarray}
% {\bfseries (B) Convergence rate of bias:}
\begin{eqnarray}
\dist\left(\widetilde{\w}_n(t), \opt_n \right) \le \frac{\log n}{\overline{\gamma}_n^2 t},
\label{eq:biasrate}
\end{eqnarray}
where $\widetilde{\w}_n(t) := \w_n(t)/\|\w_n(t)\| \in \mathbb B_m$ is the normalized version of $\w_n(t)$.
% Thus, both the margin and the bias converge at a rate of $\mathcal O(1/t)$.
\label{thm:main}
\end{restatable}
\begin{restatable}{rmk}{}
Note that it is already known via standard gradient-flow arguments (see ~\cite{GF}, for example) that the corresponding margin $\gamma_n(\w_n(t))$ in the above theorem converges to the optimal margin $\overline{\gamma}_n$ at a rate $\mathcal O(1/t)$.
\end{restatable}
\begin{restatable}{df}{}
The quantity $\dist(\widetilde{\w}_n(t),\opt_n)$ will be referred to as the bias of gradient-flow. In general, the implicit bias of an algorithm will be the rate of convergence of the (normalized) iterates produced by that algorithm and the set of max-margin classifiers.
\label{df:bias}
\end{restatable}
\begin{table*}[!h]
    \centering
    \begin{tabular}{|c|c|c|c|}
    \hline
        \emph{Paper} & \emph{Margin convergence} & \emph{Bias convergence} & \emph{Algorithm}
\\
         \hline
          ~\cite{soudry2017} & $\mathcal O(\log\log t / \log t)$ & $\mathcal O(1/\log t)$ & GD, constant stepsize\\
         \hline
          ~\cite{soudry2018} & $\widetilde{\mathcal O}(1/ \sqrt{t})$ & $\mathcal O(1/\log t)$ & GD, adaptive stepsize\\
          \hline
         ~\cite{telgarsky2019} & $\mathcal O(1/\log t)$ & $\mathcal O(1/\log t)$ & GD, constant stepsize\\
         \hline
         ~\cite{telgarsky2020} & $\mathcal O(1/t)$ & $\textcolor{blue}{\mathcal O(1/\sqrt{t})}$ & GD, aggressive stpesize\\
         \hline
         *Our paper & $\mathcal O(1/t)$ & $\textcolor{blue}{\mathcal O(1/t)}$ & GF (no stepsize)\\
         \hline
         *Our paper & $\widetilde{\mathcal O}(1/\sqrt{t})$ & $\textcolor{blue}{\widetilde{\mathcal O}(1/\sqrt{t})}$ & GD (GF discretization)\\
         \hline
         *Our paper & $\mathcal O(1/t)$ & $\textcolor{blue}{\mathcal O(1/t)}$ & GD, aggressive stepsize\\
         \hline
    \end{tabular}
    \caption{\todo{This table is now wrong. See comment after abstract.} Convergence rates established in different papers, for both the margin and the bias of gradient-descent / gradient-flow. Here, only a handful of the most representative papers are shown here for the purpose of comparison. It should be noted that in our work as well as in the works of Ji and Telgarsky above, the dependence on the sample size $n$ is a multiplicative factor $\log n$ in the numerator. The notation $\widetilde{\mathcal O}(\ldots)$ means all terms which are logarithmic in $t$ have been ignored.}
    \label{tab:comparison}
\end{table*}

The next theorem, which is a discrete-time version of Theorem \ref{thm:main} is our second main contribution.
\begin{restatable}[$\widetilde{\mathcal O}(1/\sqrt{t})$ convergence rate of the bias of gradient-descent with adaptive stepsizes]{thm}{}
Consider gradient-descent $\w_n(t+1) := \w_n(t) + \eta_t \nabla \risk_n(\w_n(t))$, with stepsizes $\eta_t = 1 / \sqrt{t + 1}$ on $-\risk_n$, where $t \in \mathbb N$ is the iteration count. Then, we have the following bound
% {\bfseries (A) Convergence rate of margin.}
% \begin{eqnarray}
% 0 \le \overline{\gamma}_n  -\gamma_n(\widetilde{\w}_n(t)) \le \frac{C\log n}{\overline{\gamma}_n \sqrt{t + 1}}.
% \end{eqnarray}
% {\bfseries (B) Convergence rate of bias.}
\begin{eqnarray}
\dist(\widetilde{\w}_n(t),\opt_n) = \widetilde{\mathcal O}(\frac{\log n}{\overline{\gamma}_n^2 \sqrt{t}}),
\label{eq:gdbiasrate}
\end{eqnarray}
\label{thm:gd}
where $\widetilde{\w}_n(t):=\w_n(t)/\|\w_n(t)\| \in \mathbb B_m$ is the normalized version of $\w_n(t)$ as usual.
\end{restatable}

Finally, we have the following theorem which improves the main result in ~\cite{telgarsky2020}.
\begin{restatable}[$\mathcal O(1/t)$ convergence rate of the bias of gradient-descent with aggressive stepsizes]{thm}{}
 Consider gradient-descent $\w_n(t+1) := \w_n(t) - \eta_t \nabla \mathcal R_n(\w_n(t))$ on the empirical risk $\mathcal R_n$, with stepsizes $\eta_t = \Theta(1 / \mathcal R_n(\w_n(t)))$. We have the bound
  \begin{eqnarray}
 \dist(\widetilde{\w}_n(t),\opt_n) = \mathcal O(\frac{\log n}{t}),   
  \end{eqnarray}
  where $\widetilde{\w}_n(t):=\w_n(t)/\|\w_n(t)\| \in \mathbb B_m$.
  \label{thm:turbo}
\end{restatable}
% \begin{restatable}[Improved rates for exponential loss: discrete-time]{thm}{} There exists a stepsize schedule such that gradient-descent on the loss $\risk_n$ has the following rates ($k$ is the iteration counter)

% %\begin{itemize}
% {\bfseries Convergence of risk:}
% \begin{eqnarray}
% \overline{\gamma}_n-\gamma_n(\widehat{\w}_n^{(k)}) % \le \frac{1}{\overline{\gamma}_n}\cdot \left(\frac{\log n}{t} + \Theta(\frac{1}{\log t})\right)
% = \mathcal O(\frac{\log n}{\sqrt{k}})+\mathcal O( \frac{1}{\log k}).
% \end{eqnarray}

% {\bfseries Convergence of model parameters:}
% \begin{eqnarray}
% \dist\left(\widehat{\w}_n^{(k)}, \arg\min\risk_n \right) % \le \frac{1}{\overline{\gamma}_n^2}\cdot\left(\frac{\log n}{t} + \Theta(\frac{1}{\log t})\right).
% = \mathcal O(\frac{\log n}{\sqrt{k}})+\mathcal O(\frac{1}{\log k})
% \end{eqnarray}
% \label{thm:main}
% \end{restatable}
\begin{restatable}{rmk}{}A few important points to note about results.
  \begin{itemize}
\item {\bfseries Improved SOTA.} Our results in Theorems \eqref{thm:gd} and \eqref{thm:turbo} are a net improvement on best known results from
  ~\cite{telgarsky2019}, where a convergence rate of $\mathcal O(1 /\log t)$ was obtained for the bias.
\item {\bfseries Parallel work ~\cite{telgarsky2020}.} The very recent work ~\cite{telgarsky2020} has obtained using an adaptive stepsize strategy, a convergence rate of $\mathcal O(1 / t)$ for the GD margin, and $\mathcal O(1/\sqrt{t})$ rate for the convergence of the bias.
Upto a logarithmic factor in $t$, this rate matches the bias rate in our Theorem \ref{thm:gd}. Finally, using the same aggressive stepsizes as in ~\cite{telgarsky2020}, our Theorem \ref{thm:turbo} establishes a $\mathcal O(1/t)$ convergence rate for the bias. % However, after a naive time-discretization which converts our GF scheme to a GD scheme, our convergence rate for the bias is $\mathcal O(1/\sqrt{t})$, which matches that in ~\cite{telgarsky2020}.
% \item {\bfseries Comparison with ~\cite{telgarsky2020}}: gradient-flow vs gradient-descent.) A minor disadvantage our work is that the margin analysis is done in continuous time (i.e gradient-flow instead of the more delicate gradient-descent done in ~\cite{telgarsky2020}). \emph{Maybe the aggressive gradient-descent stepsizes used in ~\cite{telgarsky2020}, are just an efficient discretization of gradient-flow ? % Perhaps / perhaps not.
% }
\item {\bfseries Universality of our approach.} The % technique use to establish the bias rate \eqref{eq:biasrate} is completely independent of how the
bias rates \eqref{eq:biasrate} and \eqref{eq:gdbiasrate} are obtained as follows. Once we have a margin rate, our technique can always ensure a bias rate not worst than the former. This is a desirable property, because it allows us to convert any margin rate to a bias rate which is at least as good, and without any specialized further analysis for the latter. This is unlike the approaches in the literature wherein each paper requires a separate case-by-case analysis for both the margin and bias rate.
\end{itemize}
\end{restatable}

\begin{proof}[Sketch of proof of Theorems \ref{thm:main},\ref{thm:gd}, and \ref{thm:turbo}]
  Using a standard
  gradient-flow argument (see ~\cite{GF}, for example), we know that
  \begin{eqnarray}
  \gamma_n(\widetilde{\w}_n(t)) \ge \overline{\gamma}_n - \frac{\log n}{\overline{\gamma}_n t}.
  \label{eq:firstpart}
  \end{eqnarray}
We will first establish an inequality of the form
\begin{eqnarray}
\dist\left(\w, \opt_n \right) \le  1- \frac{\gamma_n(\w)}{\overline{\gamma}_n},
\label{eq:proofmachine0}
\end{eqnarray}
which holds for all $\w \in \mathbb B_m$.
To this end, we will employ tools from nonsmooth analysis (section \ref{sec:nonsmooth}).
Combining \eqref{eq:firstpart} and \eqref{eq:proofmachine0} with $\w = \widetilde{\w}_n(t) \in \mathbb B_m$ then gives the result.

For the proof of Theorem \ref{thm:gd}, we discretize the gradient-flow \eqref{eq:gradflow} with stepsizes of order $\eta_t = 1/\sqrt{t+1}$, where $t \in \mathbb N$ is the iteration counter. We obtain the following discrete version of \eqref{eq:firstpart}
\begin{eqnarray}
  \gamma_n(\widetilde{\w}_n(t)) \ge \overline{\gamma}_n - \widetilde{\mathcal O}(\frac{\log n}{\overline{\gamma}_n \sqrt{t}}),
  \label{eq:gdfirstpart}
  \end{eqnarray}
  via arguments similar to the proof of ~\cite[Theorem 5]{soudry2018}.
  
  The bound \eqref{eq:gdbiasrate} then follows from combining \eqref{eq:gdfirstpart} and \eqref{eq:proofmachine0}.
  
  Finally, for the proof of Theorem \ref{thm:turbo}, we combine the $\mathcal O(1/t)$ margin rate from ~\cite[Theorem 4.2]{telgarsky2020} and our \eqref{eq:proofmachine0} above.
\end{proof}
% \input{results.tex}
% Inspecting the above proof, we observe that the inequality \eqref{eq:cooltool} --and its likes-- is the core ingredient which allows us to obtain our fast rates.
% \subsection{Proofs for results on neural networks}
% ...
% \subsection{Extension to other losses}
% \lorem

% \input{table.tex}
% \section{Extension to neural nets with 
% positive-homogeneous activation functions}
% \subsection{Main results for neural networks}
% ...

% \subsection{Extension to other loses}
% ...

\subsection{Proof of main results: Theorems \ref{thm:main}, \ref{thm:gd}, and \ref{thm:turbo}}
% \lorem 
% We begin with the following corollary to Theorem \ref{thm:gold} will be crucial in our prove of Theorem \ref{thm:main}.
% \begin{restatable}[Distance to max-margin solutions]{cor}{}
% For every $\w \in \mathbb B_{m}$, it holds that
% \begin{eqnarray}
% \dist(\w,\opt_n) \le 1 - \frac{\gamma_n(\w)}{\overline{\gamma}_n}.
% \end{eqnarray}
% \label{cor:maxmargin}
% \end{restatable}
% \begin{proof}
% Consider the function $g:\mathbb R^m \to \mathbb R \cup \{\infty\}$, define by $g(\w)=\gamma_n(\w) := \min_{i \in [n]}y_i\x_i^\top\w$ if $\|\w\| \le 1$ and $f(\w) = \infty$ else. The result is then obtained by taking $M=(M,\|\cdot\|)$ and $\ma_i=y_i\x_i$ for all $i \in [n]$, in Theorem \ref{thm:gold} and noting that $\arg\max g = \opt_n$ and $\max g = \overline{\gamma}_n$.
% \end{proof}
% the set of max-margin models; this is of course non-empty by compactness of $\mathbb B_m$ and continuity of the function $\gamma_n$. Also, note that $\min f = \overline{\gamma}_n$ the maximum margin for the problem. Now let $\w \in \mathbb B^m$, $\epsilon \in (0, 1)$, and set $\w_\epsilon := (1-\epsilon)\w$. Note that $\|\w_\epsilon-\w\| = \epsilon$ and  $\|\w_\epsilon\| = 1 - \epsilon < 1$. One computes
% \begin{eqnarray*}
% \begin{split}
% \dist(\w,\opt_n) &\le \|\w-\w_\epsilon\| + \dist(\w_\epsilon,\opt_n),\text{ by triangle inequality}\\
% &= \epsilon + \dist(\w_\epsilon,\opt_n),\text{ by definition of }\w_\epsilon\\
% &\le \epsilon + 1-\frac{\gamma_n(\w_\epsilon)}{\overline{\gamma}_n},\text{ by Theorem \ref{thm:gold} and the fact that }\|\w_\epsilon\| = 1-\epsilon < 1\\
% &\le \epsilon + 1 - \frac{\gamma_n(\w) - n\epsilon}{\overline{\gamma}_n},\text{ because }\gamma_n\text{ is an }n\text{-Lipschitz function}\\
% &= 1 - \frac{\gamma_n(\w)}{\overline{\gamma}_n} + \epsilon(1 + \frac{n}{\overline{\gamma}_n}).
% \end{split}
% \end{eqnarray*}
% Letting $\epsilon \longrightarrow 0^+$ then gives the result.

For proving the first part of Theorem \ref{thm:main}, we will need the
following elementary lemma proven in the appendix (see also
~\cite{telgarsky2019} for the finite-dimensional case), which gives a dual
formulation of the optimal margin $\overline{\gamma}_n$. % For completeness, a proof is given in the appendix.
% \begin{table*}[!h]
%     \centering
%     \begin{tabular}{|c|c|c|}
% \hline
%       \emph{Symbol} & \emph{Meaning } & \emph{Definition / Comment} \\
%         \hline
% %      $M$ & Model space & a Banach space\\
% %        \hline
% %      $M^\star$ & The feature space & the dual of $M$\\      
% %        \hline
%         $\w$ & Parameters of a linear model & Element of $\mathbb R^m$\\       
%         \hline
%         $\gamma_n$ & Margin function & $\min_{i \in [n]}y_i\langle  \x_i,\w \rangle$\\ 
%         \hline
%         $\overline{\gamma_n}$ & Maximum possible value of margin $\gamma_n(\w)$ & $\max_{\|\w\| \le 1}\gamma_n(\w)$\\ 
%         \hline
%         $\opt_n$ & Set of all max-margin (optimal) models & $\{\w \in \mathbb B_m \mid \gamma_n(\w) = \overline{\gamma}_n\}$ \\ 
%         \hline
%         $\risk_n$ & Empirical risk & defined in \eqref{eq:softmargin} \\
%         \hline
%         $\w_n(t)$ & Model after $t$ iterations of GF / GD on $\risk_n$ & \\
%         \hline
%       $\widetilde{\w}_n(t)$ & Normalized version $\w_n(t)$ & $\widetilde{\w}_n(t) := \w_n(t) / \|\w_n(t)\| \in \mathbb B_m$\\
%         \hline
%     \end{tabular}
    
%     \caption{Summary of key notations for margin / bias analysis, recalled here for convenience.}
%     \label{tab:my_label}
% \end{table*}
\begin{restatable}{lm}{smalllemma}
% Let $\A_n: \mathbb R^m \to \mathbb R^n$ be the linear-operator with $i$th row $y_i\x_i
% \in \mathbb R^m$. Then,
For every $\q=(q_1,\ldots,q_n) \in \Delta_{n-1}$, it holds that
$\overline{\gamma}_n \le \|\sum_{i=1}^nq_i y_i\x_i\| \le 1$.
\label{lm:smalllemma}
\end{restatable}

We are now ready to give a full detailed proof our main results.
\begin{proof}[Proof of Theorem \ref{thm:main}]
For ease of exposition, the prove is broken down into several steps.

\emph{Step 1: Uniform lower- and upper-bounds on gradient of loss.} Mindful of
the definition \eqref{eq:softmargin} of the soft-margin / exponential risk
$\risk_n(\w)$ of a linear model $\w \in \mathbb R^m$, one computes $\nabla \risk_n(\w) =
\mathbb E_{i \sim \widehat{\q}_{n,\beta}(\w)}[-y_i\x_i] = -\sum_{i=1}^n\widehat{q}_i y_i\x_i$, where $(\widehat{q}_1,\ldots,\widehat{q}_n) := \widehat{\q}_{n,\beta}$. Invoking Lemma \ref{lm:smalllemma} with $\q =
\widehat{\q}_{n,\beta}$ then gives
\begin{eqnarray}
\overline{\gamma}_n \le \|\nabla \risk_n(\w)\| \le 1,\;\forall \w \in \mathbb R^m.
\label{eq:gradbound}
\end{eqnarray}
\emph{Step 2: Lower-bounding the margin.}
We now prove the first part of the theorem. This step is elementary and
well-known (see ~\cite{GF}, for example).
So, let $t \mapsto \w_n(t)$ be a solution of the gradient-flow
\eqref{eq:gradflow}, so that $\w_n(t) = \int_0^t \nabla \risk(\w_n(\tau))d\tau$
for all $t\ge 0$. We note the following facts
\begin{itemize}
\item  {\bfseries Fact A:} $\|\w_n(t)\| = \|\int_0^t \nabla
  \risk_n(\w_n(\tau))d\tau\| \le \int_0^t \|\nabla \risk_n(\w_n(\tau))\|d\tau$, by triangle inequality.
\item {\bfseries Fact B:} $\int_0^t \|\nabla \risk_n(\w_n(\tau))\|d\tau \ge
  \overline{\gamma}_n t$, which follows from \eqref{eq:gradbound}.
    % \item {\bfseries Fact C:} $\frac{1}{\|\w_n(t)\|} =
    % \frac{1}{\|\w_n(t)-\w_0\|}\cdot \frac{\|\w_n(t)-\w_0\|}{\|\w_n(t)\|} =
    % \frac{1-\Theta(1/\log t)}{\|\w_n(t)-\w_0\|}$, by Lemma \ref{lm:telgarsky}.
\end{itemize}
Now, one computes
$\frac{d}{dt}\risk_n(\w(t)) = \langle \nabla
\risk_n(\w_n(t)),\frac{d}{dt}\w_n(t)\rangle = \|\nabla \risk_n(\w_n(t))\|^2$,
from which
\begin{eqnarray*}
\begin{split}
 \frac{\gamma_n(\w_n(t))}{\|\w_n(t)\|} &\ge \frac{\risk_n(\w_n(t))-\log
   n}{\|\w_n(t)\|},\text{ because }\risk_n(\w_n(t)) \ge \gamma_n(\w_n(t)) -
 \log n\\
&= \frac{-\log n + \int_0^t\|\nabla
  \risk_n(\w_n(\tau))\|^2d\tau}{\|\w_n(t)\|},\text{ by integrating
}\frac{d}{dt}\risk(\w(t))\text{ w.r.t }t\\
&= \frac{-\log n + \int_0^t\|\nabla
  \risk_n(\w_n(\tau))\|^2d\tau}{\int_0^t\|\nabla
  \risk_n(\w_n(\tau))\|d\tau},\text{ by {\bfseries Fact A}}\\
% &\ge \frac{-\log n}{\|\w_n(t)\|} + \frac{\overline{\gamma}_n\int_0^t \|\nabla
%   \risk_n(\w_n(\tau))\|d\tau}{\|\w_n(t)\|},\text{ by the lower-bound in
%   \eqref{eq:gradbound}}\\
% &\ge \frac{-\log n}{\|\w_n(t)\|} + \overline{\gamma}_n,\text{ by {\bfseries Fact A}}\\
% %&\ge \frac{-\risk_n(\w_0)-\log n}{\|\w_n(t)\|} + \frac{\overline{\gamma}_n\int_0^t \|\nabla \risk_n(\w_n(\tau))\|d\tau}{\|\w_n(t)\|}\\
&\ge(\frac{-\log n}{\overline{\gamma}_n t} + \overline{\gamma}_n),\text{ by
  \eqref{eq:gradbound} and {\bfseries Fact B}, provided }t\ge (\log n)/\overline{\gamma}_n^2\\
% &\gtrsim (\overline{\gamma}_n-\frac{\log n}{\overline{\gamma}_n t})\cdot (1-\Theta(\frac{1}{\log t})),\text{ for }t \ge \frac{\log n}{\overline{\gamma}_n^2}\\
% &= \overline{\gamma}_n - \frac{\log n}{\overline{\gamma}_n t} + \Theta(\frac{\overline{\gamma}_n}{\log t}) + \mathcal O\left(\frac{\log n}{t \log t}\right),\text{ by expanding}.
\end{split}
\end{eqnarray*}
Thus for $t \ge (\log n) / \overline{\gamma}_n^2$, we have that
\begin{eqnarray}
\label{eq:proofmachine}
  \gamma_n(\widetilde{\w}_n(t)) = \gamma_n(\frac{\w_n(t)}{\|\w_n(t)\|}) =
  \frac{\gamma_n(\w_n(t))}{\|\w_n(t)\|} \ge \overline{\gamma}_n - \frac{\log
  n}{\overline{\gamma}_n t},
\end{eqnarray}
from which the first part of the theorem follows.

% \emph{Step 3: Bounding the distance to set of  minimizers in terms of margin.}
% By Corollary \ref{cor:maxmargin}, for every nonzero $\w \in \mathbb R^m$ we have
% \begin{eqnarray}
% \label{eq:cooltool}
% \begin{split}
% \dist\left(\frac{\w}{\|\w\|}, \opt_n \right) &\le  1- \frac{\gamma_n(\frac{\w}{\|\w\|})}{\overline{\gamma}_n}.
% \end{split}
% \label{eq:master}
% \end{eqnarray}
\emph{Step 2: Bounding distance to set of minimizers.}
Consider the  function $g:\mathbb R^m \to \mathbb R \cup \{\infty\}$, define
by $g(\w):= \min_{i \in [n]}\langle \ma_i,\w\rangle$ if $\|\w\| \le 1$ and
$f(\w) = \infty$ else, where $\ma_i=y_i\x_i$ for all $i \in [n]$. Note that
$\arg\max g = \opt_n$ and $\max g = \overline{\gamma}_n$. Now, invoke Theorem
\ref{thm:gold} with $M=(\mathbb R^m,\|\cdot\|_2)$ to get
\begin{eqnarray}
\dist\left(\widetilde{\w}_n(t), \opt_n \right) \le  2\left(1- \frac{\gamma_n(\widetilde{\w}_n(t))}{\overline{\gamma}_n}\right)^{1/2}.
\label{eq:proofmachine}
\end{eqnarray}
Combining \eqref{eq:aggressive} and \eqref{eq:proofmachine} then gives
$$
\dist\left(\widetilde{\w}_n(t), \opt_n \right) \le \frac{\log
  n}{\overline{\gamma}_n^2 \sqrt{t}},
$$
which concludes the prove of the theorem.
\end{proof}
% Inspecting the above proof, we observe that the inequality \eqref{eq:cooltool} --and its likes-- is the core ingredient which allows us to obtain our fast rates.
% \subsection{Proofs for results on neural networks}
% ...

\begin{proof}[Proof of Theorem \ref{thm:gd}]
As explained in the proof sketch at the end of section \ref{sec:main}, the prove of Theorem \ref{thm:gd} follows from a time-discretization of the proof of Theorem \ref{thm:main}, with stepsize $\eta_t = \mathcal O(1/\sqrt{t + 1})$, where $t \in \mathbb N$ is the iteration counter.
\end{proof}

\begin{proof}[Proof of Theorem \ref{thm:turbo}] 
% Finally, for the proof of Theorem \ref{thm:turbo},
We combine the \emph{(A)} ~\cite[Theorem 4.2]{telgarsky2020} which establishes a margin rate $\gamma_n(\widetilde{\w}_n(t)) \ge \overline{\gamma}_n - \log (n) / (\overline{\gamma}_n t)$ via gradient-descent on the empirical risk $\mathcal R_n(\w) := \ell_{\exp}^{-1}(-\risk_n(\w))= (1/n)\sum_{i=1}^n\ell_{\exp}(-y_i\langle \x_i,\w\rangle)$ with aggressive stepsizes $\eta_t = \Theta(1/\mathcal R_n(\w_n(t)))$, and \emph{(B)} our inequality \eqref{eq:proofmachine} above, to get the bound
$$
\dist\left(\widetilde{\w}_n(t), \opt_n \right) = \mathcal O(\frac{\log
  n}{\overline{\gamma}_n^2 \sqrt{t}}),
$$
as claimed.
\end{proof}


==> question_to_telgarsky.tex <==
\begin{mdframed}
{\bfseries Definition (of tightness).} $b_t$ is said to a \emph{tight} bound for $a_t$ iff $a_t = \mathcal O(c_t)$ and $c_t = \mathcal O(a_t)$, i.e iff $a_t = \Theta(c_t)$, i.e $c_t$ is both an \textbf{upper bound} and a \textbf{lower bound} for $a_t$.
\end{mdframed}

Of course as usual, all of this is to be read in the sense of $t \to \infty$.

Now, your paper establishes the following three statements:

\begin{eqnarray}
\left\|\frac{w_t}{\|w_t\|}-\overline{u}\right\| \textcolor{red}{\le} \frac{2\|v_t\|}{\|w_t\|} = \mathcal O\left(\frac{\ln(n)}{\ln(t)}\right).
\end{eqnarray}
\begin{eqnarray}
\|w_t\| = \Theta(\ln(t)).
\end{eqnarray}
\begin{eqnarray}
\|v_t\| \ge \ln(n) - \ln(2).
\end{eqnarray}

Note the highlighted "$\textcolor{red}{\le}$" in (1).

The above statements imply the following statement
\begin{eqnarray}
\left\|\frac{w_t}{\|w_t\|}-\overline{u}\right\| \textcolor{red}{\le} \frac{2\|v_t\|}{\|w_t\|} = \Theta \left(\frac{\ln(n)}{\ln(t)}\right).
\end{eqnarray}

Thus, you've proved the following:
\begin{itemize}
    \item $\ln(n) / \ln(t)$ is a \textbf{tight bound} for $\frac{\|v_t\|}{\|w_t\|}$.
    \item $\ln(n)/\ln(t)$ is an \textbf{upper bound} for $\left\|\frac{w_t}{\|w_t\|}-\overline{u}\right\|$, i.e  $\left\|\frac{w_t}{\|w_t\|}-\overline{u}\right\| = \mathcal O(\ln(n)/\ln(t))$.
\end{itemize}

However,
\begin{mdframed}
\textbf{The core issue.} None of the above arguments imply in anyway that "$\ln(n) / \ln(t)$ is a tight bound (see def above) for $\left\|\frac{w_t}{\|w_t\|}-\overline{u}\right\|$. All that has been proven at this point is $\left\|\frac{w_t}{\|w_t\|}-\overline{u}\right\| = \mathcal O(\ln(n)/\ln(t))$.
\end{mdframed}

==> random_stuff.tex <==
\begin{restatable}[Ji et Telgarsky 2018 / 2019]{lm}{}
Let $t \mapsto \w_n$ be a weak-solution of the gradient-flow \eqref{eq:gradflow}. Then, for large $t>0$, it holds that $\|\w_n(t)\| = \Theta(\log t)$.
\label{lm:telgarsky}
\end{restatable}

==> results.tex <==
\begin{figure}[!htp]
    \centering
    \includegraphics[width=.8\linewidth]{dist2opt.png}
    \caption{Convergence rate of bias of gradient-descent. This toy example is on a
      separable binary classification problem on simulated data with $m=20$ features, $n=4000$ samples, and optimal margin $\overline{\gamma}_n=0.2$.
      Note that $\widetilde{\w}_n(t) := \w_n(t)/\|\w_n(t)\| \in \mathbb B_m$, where $\w_n(t) \in \mathbb R^m$ are the model parameters after $t$ steps of
      gradient-descent, as predicted by Theorem \ref{thm:turbo}.}
    \label{fig:figure}
\end{figure}

==> rkhs.tex <==
\section{Towards deep learning: the RKHS way}
Let $\mathcal H$ be a \emph{Reproducible Kernel Hilbert space -- RKHS} induced by a positive definite kernel $\kappa:\mathcal X \times \mathcal X \to \mathbb R$. The max-margin problem can be written
\begin{equation}
   \overline{\gamma}_n = \max_{\|f\|_{\mathcal H} \le 1}\gamma_n(f),
\end{equation}
where $\gamma_n(f) := \min_{i \in [n]}y_if(\x_i)$, and $T_i:\mathcal H \to \mathbb R$ is the \emph{empirical evaluation operator} defined by $T_i(f) := y_if(\x_i)$. One easily computes
$$
\nabla_f T_i (f) = T_i^\star:\mathbb R \to \mathcal H,\;q \mapsto qy_i\kappa(\cdot,\x_i).
$$

Note that $-\gamma_n(f) := \max_{i \in [n]}-T_i(f)$. Thus, if $\|f\|_{\mathcal H} < 1$ and $I(f) := \{i \in [n] \mid T_i(f) = \min_{j \in [n]} T_j(f)\}$, then we have
\begin{eqnarray*}
\begin{split}
\|\partial (-\gamma_n)(f)\|_\star &:= \inf\{\|g\|_{\mathcal H} \mid g \in \partial (-\gamma_n)(f)\}\\
&= \inf\{\|g\|_{\mathcal H} \mid g \in \conv\{-y_ik(\cdot,\x_i) \mid i \in I(f)\}\},\text{ by Lemma \ref{lm:subdiffmax}}\\
&\ge \inf_{\q \in \Delta_{n-1}}\|T^\star(\q)\|_{\mathcal H},\text{ infimum can only decrease on larger set}\\
&=\inf_{\q \in \Delta_{n-1}}\sup_{\|g\|_{\mathcal H} \le 1} \left\langle T^\star(\q),g\right\rangle_{\mathcal H},\text{ duality for RKHS norm} \\
&= \sup_{\|g\|_{\mathcal H} \le 1}\inf_{\q \in \Delta_{n-1}}\left\langle T^\star(\q),g\right\rangle_{\mathcal H},\text{ since }\inf\sup \ge \sup\inf\\
&= \sup_{\|g\|_{\mathcal H} \le 1}\inf_{\q \in \Delta_{n-1}}\left\langle\q, T(g)\right\rangle_{\mathbb R^n},\text{ duality for linear operator }T\\
&= \sup_{\|g\|_{\mathcal H} \le 1} \min_{i \in [n]}T_i(g),\text{ since min. of linear functional on simplex is attained at a vertex}\\
&=: \sup_{\|g\|_{\mathcal H} \le 1}\gamma_n(g) = \overline{\gamma}_n,\text{ by definition of maximum margin }\overline{\gamma}_n.
\end{split}
\end{eqnarray*}

==> summary.tex <==
\paragraph{Optimization, smooth margin, empirical risk.} Producing a point in $\opt$ (i.e maximizing the hard-margin function $\gamma$) is challenging due to the nonsmooth and combinatorial nature of the problem. For this reason, one usually tries to instead maximize a proxy of $\gamma$ instead, via a loss / risk functional. In this paper we will focus on the so-called exponential risk or smoothed margin function, constructed as thus. For any $\beta \in (0, \infty)$ and $\w \in \mathbb R^m$, define a Boltzman
distribution $\widehat{\q}_{n,\beta}(\w)
% = (q_1,\ldots,q_n)
\in \Delta_{n-1}$ by
setting $q_i \propto e^{-\beta y_i\x_i^\top\w}$ for each $i \in [n]$. Also define
the smooth margin at temperature $\beta$, of a model $\w$ 
\begin{eqnarray}
\risk(\w) := -\ell_{\exp}^{-1}(\mathcal R) = -\frac{1}{\beta}\log(\frac{1}{n}\sum_{i=1}^n e^{-\frac{1}{\beta}y_i\x_i^\top\w}),
% = \frac{1}{\beta}\log(\mathbb E_{(\x,y) \sim \widehat{P}} e^{-\beta y\x^\top \w}),
\label{eq:softmargin}
\end{eqnarray}
where $\ell_{\exp}(u) := e^{\beta u}$ is the exponential loss, and $\mathcal R(\w) := \frac{1}{n}\sum_{i=1}^n\ell_{\exp}(-y_i\x_i^\top\w))$ is the empirical risk.
Note that
\begin{eqnarray}
\gamma(\w) \le \risk(\w) \le \gamma(\w) + \log n.
\end{eqnarray}

\begin{mdframed}
{\bfseries Implicit bias.} One is then interested in the convergence of approximate minimizers of $-\risk$ via, say gradient-descent, to a point in $\opt$. This is the so-called \emph{implicit bias} of gradient-descent. See ~\cite{soudry2017} and ~\cite{telgarsky2019}, for example.
\end{mdframed}

\paragraph{Summary of main contributions.} Our main contributions can be summarized as follows.
\begin{itemize}
\item For exponential-tailed functions (as defined in ~\cite{soudry2017}), including the exponential loss function $\ell_{\exp}$ in the definition of the smoothed margin $\risk$ defined above, we show in Theorem \ref{thm:main} that gradient-flow on the empirical risk produces a sequence of iterates whose margin and bias both converge at a rate of $\mathcal O(\log n/t)$, where $n\ge 2$ is the number of samples in the training sample, and $t>0$ is time (continuous). Via time-discretization, we show in Theorem \ref{thm:gd} that this leads to a $\widetilde{\mathcal O}(\log n/\sqrt{t})$ bias convergence rate in the case of gradient-descent, after $t$ iterations (discrete). % Here $\widetilde{\mathcal O}(\ldots)$ means we are hiding terms which are only logarithmic in the iteration count $t$.
\item An important by-product of our technique is that it allows us to convert any convergence rate for the margin, to a convergence rate for the bias which is at least as good as the former. In particular, using our methods we derive a convergence rate of $\mathcal O(\log n / t)$ for the bias, directly from the $\mathcal O(\log n / t)$ margin rate that has been very recently established in ~\cite{telgarsky2019}. We believe our methods provide a powerful new way to derive convergence rates for the implicit bias of gradient-flow / gradient-descent.
\end{itemize}

==> table.tex <==
\begin{table*}[!htbp]
    \centering
\begin{tabular}{|c|c|c|}
  \hline
  {\bfseries Quantity} & {\bfseries Linear version} & {\bfseries Nonlinear version}\\
  \hline
Model instance & vector $\w$ in $\mathbb R^m$  & function $h$ in RKHS $\mathcal H$ \\
  \hline
    Model prediction & $\sign(\x^\top \w) \in \{\pm 1\}$ & $\sign(h(\x)) \in \{\pm 1\}$ \\
  \hline
% Margin of a sample & $y_i\x_i^\top \w$ & $y_i h(\x_i)$ & \\
 % \hline
  Margin of a model & $\gamma_n(\w) := \min_{i \in [n]}y_i\x_i^\top \w$ & $\gamma_n(h) := \min_{i \in [n]} y_i h(\x_i)$\\
  \hline
Model norm constraint & $\|\w\| \le 1$ & $\|h\|_{\mathcal H} \le 1$\\
  \hline
  Maximum margin & $\overline{\gamma}_n := \max_{\|\w\| \le 1}\gamma_n(\w)$ & $\overline{\gamma}_n := \max_{\|h\|_{\mathcal H} \le 1}\gamma_n(h)$\\
  \hline
  Empirical loss (exponential) & $-\frac{1}{\beta}\log(\sum_{i=1}^n e^{-\frac{1}{\beta}y_i\x_i^\top \w})$ & $-\frac{1}{\beta}\log(\sum_{i=1}^n e^{-\frac{1}{\beta}y_ih(\x_i)})$\\
  \hline
  Empirical loss (logistic) & $\sum_{i=1}^n \log(1+e^{-y_i\x_i^\top \w})$ & $\sum_{i=1}^n \log(1+e^{-y_ih(\x_i)})$\\
  \hline
  % Large $\epsilon$ & $\epsilon = \omega(1)$ & $p(\epsilon) = 1-o(1) \to 1$ & Definitely vulnerable!\\
% \hline
\end{tabular}
\caption{Correspondence between linear and nonlinear (i.e function space) large-margin models.
}
\label{table:summary}
\end{table*}
...
